Blind Biological Sequence Denoising with Self-Supervised Set Learning

Biological sequence analysis relies on the ability to denoise the imprecise output of sequencing platforms. We consider a common setting where a short sequence is read out repeatedly using a high-throughput long-read platform to generate multiple subreads, or noisy observations of the same sequence. Denoising these subreads with alignment-based approaches often fails when too few subreads are available or error rates are too high. In this paper, we propose a novel method for blindly denoising sets of sequences without directly observing clean source sequence labels. Our method, Self-Supervised Set Learning (SSSL), gathers subreads together in an embedding space and estimates a single set embedding as the midpoint of the subreads in both the latent and sequence spaces. This set embedding represents the "average" of the subreads and can be decoded into a prediction of the clean sequence. In experiments on simulated long-read DNA data, SSSL methods denoise small reads of $\leq 6$ subreads with 17% fewer errors and large reads of $>6$ subreads with 8% fewer errors compared to the best baseline. On a real dataset of antibody sequences, SSSL improves over baselines on two self-supervised metrics, with a significant improvement on difficult small reads that comprise over 60% of the test set. By accurately denoising these reads, SSSL promises to better realize the potential of high-throughput DNA sequencing data for downstream scientific applications.

==> sim_light.tex <==


\textbf{Sim Antibody:} \quad
To evaluate the ability of our model to distinguish genetic variations in similar source sequences, we use a dataset of 62 light chain antibody sequences.

\subsection{Sim Antibody}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[scale=0.42]{fig/light_edit_hist.png}
         \label{fig:sim_q_vs_con}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \scalebox{0.65}{
            \input{tikz/sim_light}
         }
         \label{fig:sim_rep_per_num}
    \end{subfigure}
        \caption{Results on Sim Random data. Our denoising method achieves almost 4 base pair lower edit distance on average compared to MSA consensus. We perform particularly well in the low subread setting, beating the MSA consensus by a large margin when there are less than 11 subreads.}
        \label{fig:sim_res}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Results on Sim Antibody data are shown in Figure...

==> tikz/extra.tex <==
\addplot+[mark=*, error bars/.cd, y dir=both, y explicit,] table [x=x, y=y,y error=error, col sep=comma] {
x,  y,      error
%1, 33.0, 0.0
%2, 33.0, 0.0
3, 58.542194092827, 12.19338342730868
4, 65.33271028037383, 12.534123708515152
5, 51.0446247464503, 10.430978423103058
6, 49.35796766743649, 8.916279194187481
7, 40.94237288135593, 7.242066457360352
8, 43.47286821705426, 7.97824320521429
9, 38.21739130434783, 6.399885789781192
10, 37.358381502890175, 6.445763203564095
11, 34.68835616438356, 5.678799919937413
12, 34.136842105263156, 5.195025676749519
13, 32.049549549549546, 4.684868759377351
14, 32.38121546961326, 5.058058573571815
15, 30.54248366013072, 3.8399123902461216
16, 30.085714285714285, 4.761180897363065
17, 29.12, 4.101901997854166
18, 28.76, 3.507477726230061
19, 29.208333333333332, 3.8511812762089273
20, 30.0, 4.3094580368566735
21, 28.833333333333332, 3.1841621957571333
22, 26.0, 0.0
};
\addlegendentry{MAFFT}

\addplot+[mark=*, error bars/.cd, y dir=both, y explicit,] table [x=x, y=y,y error=error, col sep=comma] {
x,  y,      error
%1, 33.0, 0.0
%2, 33.0, 0.0
3, 54.620253164556964, 11.461883775485736
4, 57.54579439252336, 10.966271828971067
5, 44.8235294117647, 8.990827764568564
6, 42.006928406466514, 7.064692683558087
7, 35.328813559322036, 5.887391032420872
8, 36.69767441860465, 6.322844825289834
9, 32.869565217391305, 4.9773779357521075
10, 32.04624277456647, 4.956825187664026
11, 30.339041095890412, 4.694588451008089
12, 29.856140350877194, 3.988185074796297
13, 28.346846846846848, 3.9503066324093914
14, 28.49171270718232, 3.760243886134075
15, 27.22875816993464, 3.2509359778943496
16, 27.038095238095238, 3.4556339354294474
17, 26.933333333333334, 3.3638602164114304
18, 26.82, 2.861398259592677
19, 26.791666666666668, 3.3662437853224807
20, 27.285714285714285, 4.164965639175215
21, 27.333333333333332, 2.2852182001336816
22, 25.0, 0.0
};
\addlegendentry{MUSCLE}

\addplot+[mark=*, error bars/.cd, y dir=both, y explicit,] table [x=x, y=y,y error=error, col sep=comma] {
x,  y,      error
%1, 33.0, 0.0
%2, 33.0, 0.0
3, 47.28270042194093, 9.737061971153528
4, 47.82056074766355, 9.31291674917965
5, 37.59229208924949, 7.637455837067903
6, 35.64203233256351, 5.987190909936495
7, 30.728813559322035, 5.163859115549133
8, 32.6124031007752, 5.167444418859858
9, 29.51304347826087, 4.2399724173110975
10, 28.898843930635838, 4.390432167482018
11, 27.763698630136986, 3.893573562584685
12, 27.67719298245614, 3.6032644820592967
13, 26.463963963963963, 3.399265760486096
14, 26.85635359116022, 3.4290481527807857
15, 26.07843137254902, 3.123868499497541
16, 25.885714285714286, 2.925468739696046
17, 25.613333333333333, 2.612244671201804
18, 25.82, 2.76181100005051
19, 25.666666666666668, 2.8819360776317637
20, 26.5, 3.736881817008094
21, 26.333333333333332, 2.6246692913372702
22, 24.0, 0.0
};
\addlegendentry{T-Coffee}
